CoVer-ability: Consistent Versioning for Concurrent Objects

An object type characterizes the domain space and the operations that can be invoked on an object of that type. In this paper we introduce a new property for concurrent objects, we call coverability, that aims to provide precise guarantees on the consistent evolution of an object. This new property is suitable for a variety of distributed objects including concurrent file objects that demand operations to manipulate the latest version of the object. We propose two levels of coverability: (i) strong coverability and (ii) weak coverability. Strong coverability requires that only a single operation can modify the latest version of the object, i.e. "covers" the latest version with a new version, imposing a total order on object modifications. Weak coverability relaxes the strong requirements of strong coverability and allows multiple operations to modify the same version of an object, where each modification leads to a different version. Weak coverability preserves consistent evolution of the object, by demanding any subsequent operation to only modify one of the newly introduced versions. Coverability combined with atomic guarantees yield to coverable atomic read/write registers. We also show that strongly coverable atomic registers are equivalent in power to consensus. Thus, we focus on weakly coverable registers, and we demonstrate their importance by showing that they cannot be implemented using similar types of registers, like ranked-registers. Furthermore we show that weakly coverable registers may be used to implement basic (weak) read-modify-write and file objects. Finally, we implement weakly coverable registers by modifying an existing MWMR atomic register implementation.

==> figures/model-v2.tex <==
We consider a distributed system composed of $n$ \emph{asynchronous} processes
with identifiers from a set $\idSet=\{p_1,\ldots,p_n\}$, 
each of which represents a sequential thread of control. Processes
may interact with a set of shared objects $\mathcal{O}$, where each 
object represents a shared data structure. A process invokes an 
operation  


Processes communicate
by exchanging \emph{messages} through \emph{reliable},
%\footnote{Reliability is not necessary for the correctness of the algorithms we present. It is just used for simplicity of presentation.}, 
\emph{asynchronous} channels. A subset of 
processes may fail by \emph{crashing}. 
%
A distributed algorithm $A$ is defined over a set of \emph{states}
and \emph{actions}. Each state of $A$ is a vector containing the states
of each participating process. An execution of $A$ is an alternate sequence of states and actions starting with the initial state. 
A transition from a state $\st$ to a state $\st'$ as a result 
of an action $\acts$ is called a \emph{step} of $A$.   
%
%
%A distributed algorithm $A$ is defined over a set of \emph{states}, $\stateSet{A}$,
%and \emph{actions}, $\actionSet{A}$. Each state of $A$ is a vector containing the states
%of each process $\pr\in\idSet$ that participates in the distributed algorithm. Initially, all processes start at a predefined initial state. The vector of all the initial states  %that together compose the initial 
%is the state $\st_0$, the initial state of $A$. 
%An \emph{execution} $\EX$ of $A$ is an
%alternate sequence
%$\st_0,\acts_1,\st_1,\ldots,\st_{n-1},\acts_{n-1},\st_n$ 
%of \emph{states} and \emph{actions}, s.t. 
%$\st_0$ is the initial state of $A$ and $\st_i\in \stateSet{A}$ and $\acts_i\in \actionSet{A}$, for $1\leq i \leq n$. 
%A triple $\tup{\st_i,\acts_{i+1},\st_{i+1}}$ is called 
%a \emph{step} and denotes the transition from state $\st_i$ 
%to the state $\st_{i+1}$ as a result of the execution of 
%action $\acts_{i+1}$.

\remove{
An algorithm $A$ is defined over a set of \emph{sates}, $\stateSet{A}$,
and \emph{actions}, $\actionSet{A}$ and is the composition 
of the algorithms $A_\pr$ assigned to each process $\pr\in\idSet$. An algorithm $A_\pr$ is in turn defined over the set of states $\stateSet{A_\pr}$ and actions $\actionSet{A_\pr}$. A state $\st\in\stateSet{A_\pr}$ is defined by the value of the state variables at $\pr$. Each state $\st\in\stateSet{A}$ at a time $t$ is a vector containing the state
of each process $\pr\in\idSet$, denoted by $\st[\pr]$, at time $t$. We refer to the state $\st_0$ as 
the initial state of the algorithm that contains the initial
states $\st_0[\pr], \forall \pr\in\idSet$. The set of actions 
of $A$ is the union of the actions performed by each process; more formally $\actionSet{A}=\bigcup_{\pr\in\idSet}\actionSet{A_\pr}$.
  
An \emph{execution} $\EX$ of a distributed algorithm $A$ is an
alternate sequence
$\st_0,\acts_1,\st_1,\ldots,\st_{n-1},\acts_{n-1},\st_n$ 
of \emph{states} and \emph{actions}, s.t. 
$\st_0$ is the initial state of $A$ and $\st_i\in \stateSet{A}$ and $\acts_i\in \actionSet{A}$, for $1\leq i \leq n$. 
A triple $\tup{\st_i,\acts_{i+1},\st_{i+1}}$ is called 
a \emph{step} and denotes the transition from state $\st_i$ 
to the state $\st_{i+1}$ as a result of the execution of 
action $\acts_{i+1}$.
}

An implementation of a \emph{traceable} atomic read/write shared 
%object offers two operations: \emph{update} and \emph{read}. An \emph{update} is requested at a process $\pr$ when
%the $\act{update}_\pr(v)$ action occurs and a \emph{read} is requested when the action $\act{read}_\pr$ occurs. The process 
%$\pr$ obtains the result of an update or read operation when 
%the $\act{update-ack}$ or $\act{read-ack}(v)$  actions occur 
%respectively. The step that contains the $\act{update}_\pr(v)$ or $\act{read}_\pr$ actions is called a \emph{invocation} step
%and the step that contains either the $\act{update-ack}$ or the $\act{read-ack}(v)$ action is called a \emph{response} step.
object offers two operations: \emph{read} and \emph{write}. A process $\pr$ \emph{invokes} a \emph{write} (resp. \emph{read}) operation when it issues 
a $\act{write}_\pr(v)$ (resp. $\act{read}_\pr$) request. %and a \emph{read} is requested when the action $\act{read}_\pr$ occurs. 
Similarly, a process 
$\pr$ \emph{responds} to a write or a read operation when 
the $\act{write-ack_\pr}$ or $\act{read-ack}_\pr(v)$  actions occur respectively. The step that contains the $\act{write}_\pr(v)$ or $\act{read}_\pr$ actions is called an \emph{invocation} step
and the step that contains either the $\act{write-ack}_\pr$ or the $\act{read-ack}_\pr(v)$ action is called a \emph{response} step.
An operation $\op$ is \emph{complete} in an execution $\EX$ if $\EX$ contains the 
invocation and a matching response step for $\op$; otherwise
$\op$ in \emph{incomplete}.
An operation $\op$ \emph{precedes} an operation $\op'$ (or 
$\op'$ \emph{succeeds} $\op$) in 
an execution $\EX$, denoted by $\op\bef\op'$, if the response 
step of $\op$ appears before the invocation step of $\op'$ 
in $\EX$; if none of the operations precedes the other, the two operations are \emph{concurrent}.\vspace{-.5em}
%, denoted by $\op\conc\op'$. 
%We say that $\op$ is the \emph{last preceding} operation of type $T$ to an operation $\op'$, denoted by $\op\imbef\op'$, 
%if $\op\bef\op'$ and there is no operation $\op''$ of type $T$ s.t. $\op\bef\op''\bef\op$.  

\begin{definition}%[Atomicity.]
\label{def:atomic}
{\rm An execution $\EX$ is \emph{atomic} \cite{Lynch1996} if every 
\emph{read} and \emph{write} operation in $\EX$ is \emph{complete}
and there is a partial ordering $\prec$ on all operations 
$\Pi$ in $\EX$ such that: {\bf A1.} For any pair of operations $\op_1,\op_2\in\Pi$, if $\op_1\bef\op_2$ in $\EX$ then it cannot hold that $\op_2\prec\op_1$, {\bf A2.} If $\op\in\Pi$ is a \emph{write} operation and $\op'$ any operation in $\Pi$,
then either $\op\prec\op'$ or $\op'\prec\op$, and {\bf A3.} If $v$ is the value returned by a \emph{read} $\rd$ then $v$ is the value written by the last preceding \emph{write} according to $\prec$
(or the initial value $v_0$ if there is no such a write).}\vspace{-.5em}
\end{definition}

%Having defined atomicity we need 
It now remains to specify \emph{traceability}. We first define the \emph{revision} relation 
between two values $v$ and $v'$.%\vspace{-.5em}

%\nn{The function needs not to be trivial otherwise 
%any change on the value of the atomic object can 
%be considered as a change on the previous value.}
\begin{definition} %[Revision.]
\label{def:depend}
{\rm A value $v'$ is a \emph{revision} ( or revises) a value $v$, denoted by $v\dep v'$, if there is a function $\mathcal{F}$ s.t. $v'=\mathcal{F}(v)$.}\vspace{-.5em}  
\end{definition}

The \emph{revision} relation is \emph{transitive} since 
if $v'=\mathcal{F}(v)$ and 
$v''=\mathcal{G}(v')$, then $v''=\mathcal{G}(\mathcal{F}(v))$.
Hence, if a value $v\dep v'$ and $v'\dep v''$, then 
$v\dep v''$.  
We can now extend the definition of atomicity to 
define the \emph{traceable} atomic shared objects.\vspace{-.5em} 

\begin{definition} %[Traceability.]
\label{def:vdependability}
{\rm 
An execution $\EX$ of a shared object implementation $A$ satisfies {\bf traceable atomicity} if $\EX$ satisfies properties {\bf A1} - {\bf A3} and the following properties:} \vspace{.3em}
%\begin{itemize}
%\item 

{\rm \noindent\T {\bf A4. Validity:} For each \emph{write} $\wrt(v)$ there exists a value $v'$ s.t. $v'\dep v$ and $\wrt(v')\prec\wrt(v)$ or $v'=v_0$}, 
%and (ii) if there exists 
%a write operation $\wrt(v')\bef\wrt(v)$, then $\forall v''$,
%s.t. $v''\dep v'$, it holds that $v''\dep v$.} 
\vspace{.3em}

{\rm \noindent\T {\bf A5. Continuity:} For each \emph{write} $\wrt(v)$ if there exists 
a write operation $\wrt(v')\bef\wrt(v)$, then $\forall v''$,
s.t. $v''\dep v'$, it holds that $v''\dep v$.} \vspace{.3em}

%\item 
{\rm \noindent\T {\bf A6. Consolidation:} If $\op(v)$ is a \emph{read} 
that returns $v$ or a \emph{write} that writes $v$ and $\nexists \op'$ s.t. $\op'$ is \emph{concurrent} with $\op$,
then $\forall \wrt(v')$, s.t. $\op(v)\bef\wrt(v')$, it holds that $v\dep v'$.
We refer to $\op(v)$ as a \emph{barrier} operation.}\vspace{-.5em} 
%$v\dep v'$ where $v'$ is the value written by either the last preceding write operation according to $\bef$ or the last
%preceding write operation according to $\prec$ (or $v'=v_0$ 
%if there is no such a write).  
%\end{itemize}
%
\end{definition}

By 
%Definition \ref{def:vdependability} and 
\emph{continuity} each value written on the shared object 
%must depend on 
revises a version written by a preceding write operation. %according to $\prec$. 
Continuity allows two \emph{writes} to depend 
on different values creating this way two different version "branches". \emph{Consolidation} defines through a solo operation (i.e.,
that is not concurrent with any other operation) a dominating
version eliminating any potential branches and forcing any 
subsequent write operation to revise that version of the object. Note that starting from a value $v$ 
%that satisfies \emph{consolidation}
 one may
obtain a chain of \emph{versions} of the object 
%starting from $v$ 
all the way to the initial value of the object $v_0$.

%the value written by write operation $\wrt$  
%should depend on the value written by the last 
%write operation $\wrt_1$ s.t. $\wrt_1\bef\wrt$ or on 
%the value written by a \emph{concurrent} write operation
%where $\wrt_2$ s.t. $\wrt_2\nrightarrow\wrt$ and $\wrt\nrightarrow\wrt_2$.  

\subsection{Examples of Traceability}

The easiest way to visualize the impact of the \emph{continuity} and \emph{consolidation}  properties
on the \emph{read} and \emph{write} operations is by examining  some execution fragments.
%
Consider the execution fragments that appear in Figure \ref{fig:examples}. Each fragment is placed on top of
a right arrow that denotes the passing of the real time. 
The smaller lines with the dotted ends denote the 
execution interval of a single operation. 
%The starting dot 
%denotes the time of the invocation of the operation and 
%the ending dot denotes the time of the response of the operation. 
Operations are applied on 
a single shared object thus we omit any references to the object's identifier. We use $W_\pr(v)$ to 
denote that process $\pr$ writes value $v$ on the object 
and we use $R_\pr(v)$ to denote that the process $\pr$ 
performs a read operation that returns the value $v$. Notice 
that we do not examine the feasibility of each example 
but the conditions that need to be satisfied for an execution
to preserve \emph{traceability}.

\begin{figure}
	\begin{center}
		\begin{subfigure}[b]{0.45\textwidth}		
			\includegraphics[width=\textwidth]{figures/ex1.png}
			\caption{Execution $\EX_1$}
            \label{fig:ex1}		
		\end{subfigure}
		~
		\begin{subfigure}[b]{0.45\textwidth}
			\includegraphics[width=\textwidth]{figures/ex2.png} 
			\caption{Execution $\EX_2$}
            \label{fig:ex2}		
		\end{subfigure}
		\\
		~
		\begin{subfigure}[b]{0.45\textwidth}
			\includegraphics[width=\textwidth]{figures/ex3.png}
			\caption{Execution $\EX_3$}
            \label{fig:ex3}
		\end{subfigure}		
		~		
		\begin{subfigure}[b]{0.45\textwidth}
			\includegraphics[width=\textwidth]{figures/ex4.png}
			\caption{Execution $\EX_4$}
            \label{fig:ex4}
		\end{subfigure}
	\end{center}
	\vspace{-0.7cm}
	 \caption{Execution Examples \vspace{-0.6cm}}\label{fig:examples}
\end{figure} 
%Consider an execution with two non-concurrent write operations,
%$\wrt(v)$ and $\wrt(v')$ such that $v'\neq\mathcal{F}(v)$. 
%In an atomic register implementation every server receiving 
%the value $v'$ replaces $v$ as $\wrt(v)\bef\wrt(v')$.

It is easy to observe that all executions presented in Figure 
\ref{fig:examples} preserve \emph{atomicity} as they satisfy
properties {\bf A1}-{\bf A3} of Definition \ref{def:atomic}.
%They do not necessarily satisfy \emph{v-dependability}. Notice 
%that if the values $v'$ and $v''$ in all the examples do not 
%\emph{depend} on $v$ then v-dependability is violated. 
%Therefore  atomic read/write implementations are not \emph{v-dependable}.
%
Let us investigate 
%each execution separately to see 
when \emph{traceability} is satisfied. 
Notice that if the values $v'$ and $v''$ do not 
\emph{revise} $v$ then \emph{consolidation} is violated
in all the examples. 
Figures \ref{fig:ex1} and \ref{fig:ex2} present two executions that contain three \emph{barrier} operations.
In both executions the \emph{barrier} operation $W_p(v)$
precedes all other operations. Thus \emph{consolidation}
is satisfied only
%execution $\EX_1$ that contains 
%no concurrency. Since $W(v)$ is the last preceding write 
%operation of $W(v')$ then $\EX_1$ is \emph{v-dependable} 
if $v'$ \emph{revises} $v$ (e.g., $v\dep v'$). Execution $\EX_2$ in Figure \ref{fig:ex2} contains a hidden write (i.e., a write that is never read). 
%The value $v'$ should according to 
%Definition \ref{def:vdependability} depend on $v$ and hence $v'\dep v$. Notice that 
Since $v\dep v'$ then $v$ can be obtained by $R$ 
by applying the reverse of the function $\mathcal{F}$ that was used 
to derive $v'$ from $v$. Note here that executions like $\EX_2$ 
may not be possible if the two writes are invoked by different processes. 
%In order for a value to depend on another value
%a process needs to obtain that value before writing. So 
A \emph{read} might have been necessary from $q$ preceding the write operation $W_q(v')$ in order for $v'$ to be a revision of $v$. 

Execution $\EX_3$ in Figure \ref{fig:ex3} is slightly more complex, having two concurrent \emph{writes}. According to the values returned by the read operations $R_p(v')$ and $R_p(v'')$ it follows that write $W_q(v')$ precedes $W_z(v'')$ 
according to $\prec$. So \emph{continuity} is preserved only if 
both $v'$ and $v''$ \emph{revise} $v$ or if $v\dep v'$ and $v'\dep v''$. Notice that $R_p(v'')$ is a \emph{barrier} operation and 
thus by \emph{consolidation} any write succeeding this operation should write a value $\hat{v}$ such that
$v''\dep \hat{v}$.
%V-dependability is violated in this case if $v'\dep v''$,
%as $ W_z(v'')$ is \emph{concurrent} with $W_q(v')$ but $W_q(v')\prec W_z(v'')$.

%In execution 4 it appears that we can make \emph{consolidation}
%a bit stricter by saying that $v'\dep v$ if $w(v)\bef w(v')$ 
%and $w(v)$ is the last preceding operation of $w(v')$ 
%according to $\prec$. We can also leave the definition 
%more general for the BA and remove $\EX_4$ from the examples.
Lastly execution $\EX_4$ in figure \ref{fig:ex4} presents 
a scenario where a write operation is concurrent with 
two write operations. This execution is v-dependable in the 
following cases: (i) $v'\dep v$, $v''\dep v$, and $v'''\dep v'$, (ii)  $v''\dep v$, $v'\dep v''$, and $v'''\dep v'$, and
(iii) $v'\dep v$, $v''\dep v$, and $v'''\dep v''$. V-dependability
is violated if $v'\dep v''$, $v''\dep v$, and $v'''\dep v''$
as in this case $W_q(v')$ is both the last write s.t. $W_q(v')\bef W_z(v''')$ and the last preceding write in the partial 
order s.t. $W_q(v')\prec W_z(v''')$. So $v'''$ could only 
depend on $v'$ and not on $v''$.


\subsection{Traceability implies weak RMW registers.}

A shared object satisfies atomic \emph{read-modify-write} (RMW) semantics if 
a process can atomically \emph{read} and \emph{modify} 
the value of the object using some 
function $\mathcal{F}$, and then \emph{write} the new value on 
the object. 
%For atomic RMW objects all operations need 
%to be executed atomically, i.e. without any operation 
%overlapping any stage of the RMW operation. 
%
We claim that traceable atomic objects %results in objects that 
guarantee a weak version of RMW semantics. Consider the 
execution $\EX_1$ of figure \ref{fig:ex1}. Here the 
process $q$ performs a read operation that obtains 
$v$, it applies a local computation obtaining $v'=\mathcal{F}(v)$, and writes $v'$ on the register. This execution 
is identical to an atomic RMW operation of $q$ on 
the shared object that modifies the value $v$ of the object 
to $v'$ using the same function $\mathcal{F}$. Notice that a read/write atomic register does not guarantee this behavior as $v'$ may be independent of $v$. So we say that 
v-dependability property provide \emph{atomic RMW guarantees 
when no concurrency exists in the system}. 

Consider now execution $\EX_3$ in Figure \ref{fig:ex3}, which 
contains a number of \emph{concurrent} write operations. 
According to \emph{traceability} the values $v'$ and $v''$ 
should both revise $v$ but also one may revise the other. Let w.l.o.g. 
$v\dep v'$ and $v'\dep v''$ (by transitivity $v\dep v''$). In this case the operations 
satisfy atomic RMW semantics as such execution is identical 
with an execution where $q$ reads and modifies $v$ to $v'$  and writes $v'$,
and $z$ reads and modifies $v'$ to $v''$ and writes $v''$.
The only problematic case is when none of $v'$ and $v''$ revise the other. 
%depend on $v$. 
In this case both processes seem to read and modify $v$ and yet write a different value on the object, violating the 
atomicity of the RMW semantic. However after the completion
of both write operations, any succeeding operation 
witnesses a single value on the atomic object,
and thus a single RMW operation to take effect. 
%Thus, only 
%a single write operation among the concurrent ones 
%manages to read,modify and write the value of the last write 
%that precedes according to $\bef$ all the concurrent write 
%operations. 
In $\EX_3$ the \emph{barrier} read operation $R_p(v'')$ denotes that process $z$ had succesfully 
modified the value of the object from $v$ to $v''$. 
%read and modified $v$ to $v''$ and wrote $v''$. 
And hence, the \emph{weakness} of the RMW object is that in case where two or more
concurrent RMW operations try to modify the same object value, 
\emph{only a single} of those operations
is guaranteed to succeed. 
%and reads, modifies and writes the
%value written by the last non-concurrent write operation. 
  
%whereas some inconsistencies may 
%appear in the case of \emph{concurrent} operations. 
%Those inconsistencies can be quantified and provide 
%specific guarantees on the behavior of the shared object. 
%The dependence of each written value on a preceding \emph{write} operation implies that a writer performs 
%a successful write operation only when is aware of the latest
%value written on the object. enforces a writer process to acquire the latest written value before, modifying that to the new value is about to write on the object. This  

==> impossibility.tex <==
We now show that is impossible to implement weak traceable 
read/write registers using ranked-registers \cite{GD05}. Before proceeding
to the result we present some definitions and preliminaries. 

%\begin{definition}
%\label{def:revise}
%An operation $\op$ invoked by process $\pr_i$ \emph{revises} the version $ver$ of a traceable register 
%in an execution $\EX$, if the step $\tup{(\val{},ver), (\op,ver)_{p_i}, (\val'{}, ver')}$ 
%s.t. $ver'>ver$ appears in $\EX$.
%\end{definition}

\begin{definition}
\label{def:witness}
An operation $\trop{ver'}{*,*}_{\pr_i}$ invoked by process $\pr_i$, {\bf \emph{witnessed}} a version of a traceable register  
$ver$ in an execution $\EX$, if $ver'>ver$.
\end{definition}

We want to use rank-registers to implement the operations of
a traceable register. As in Section \ref{sec:model}, 
we denote by $\trw{ver, v}{ver', flag}$ the 
traceable write operation that tries to revise version $ver$ 
and write value $v$ on the register, and returns version $ver'$ with 
a $flag\in[mod, unchg]$. Similarly we denote by 
$\rrw{r, v}{r_h, res}$ a write operation on a ranked-register that 
uses rank $r$ and tries to write $v$ on the register. The rank 
$r'$ is the highest rank observed by an operation and $res\in[abort, commit]$.
For the rest of the section we avoid the reference to the 
value of the register. Trivially we can associate a value with 
a version or rank. 
%Since the version defines the possible transitions on a traceable
%register   
%Traceability does not impose any 
%restrictions on the behavior of read operations but rather
%only restricts the behavior of write operations. In the 
%lemmas and proofs that follow we consider executions that 
%contain write operations. 

We begin with a lemma that shows that a traceable write operation 
revises a the traceable register only if the write operation 
on the rank register commits. 

\begin{lemma}
\label{lem:commit}
Suppose there exists an algorithm that implements a traceable register
using ranked-registers. Then, in any execution $\EX$, 
a traceable write operation $\trw{ver}{ver',mod}_{\pr_i}$ \emph{revises} a version $ver$ 
iff it performs a write operation $\rrw{r}{r_h, commit}_{\pr_i}$ 
on some shared ranked-register.% and that write \emph{commits}. 
\end{lemma}


\begin{proof}
We will investigate the two directions separately. 
Let the traceable register be implemented by $k$ 
ranked registers each with a highest rank $r_1, r_2,\ldots,r_k$ 
respectively at the end of some execution fragment $\EX$. 
For the rest of the proof we will construct extensions of $\EX$.  
Also, let the state of the traceable object be $(v, ver)$ at the 
end of $\EX$.

\noindent{\bf Direction 1:} 
Let us begin with the direction that 
a write $\trw{ver}{ver',mod}_{\pr_i}$ \emph{revises} a version $ver$ then 
a write operation $\rrw{r}{*,commit}_{\pr_i,j}$ on some ranked register $j$ 
\emph{commits}. 
Assume to derive contradiction that we extend $\EX$ 
with a write operation $\wrt_1 = \trw{ver}{ver',mod}_{\pr_i}$
%. According to traceability 
%since no other operation is concurrent with this write, and since 
%it uses the same version as the version of the latest state of the 
%object, then it may 
that revises the traceable register, and 
all the write operations performed during $\wrt_1$ on the ranked 
registers abort. From that it follows that for each 
write operation $\rrw{r}{r_j,abort}_{\pr_i,j}$ performed 
by $\pr_i$ on some register $j$, $r_j > r$. 
Let the new execution be $\EX'$. 
%and let the last 
%step in $\EX'$ be $\tup{(v,ver), \trw{v_1, ver}_{\pr_i}, (v_1, ver')}$.

We extend $\EX'$ with a another write operation 
$\wrt_2 = \trw{ver'}{ver'',mod}_{\pr_z}$ by process $\pr_z$ to obtain 
execution $\EX''$. Since the last value of the register is associated with $ver'$ 
in $\EX'$ and since $\wrt_2$ 
is not concurrent with any other operation then $\wrt_2$ 
revises the value of the register to preserve traceability. 
Note however that for any write operation $\rrw{r'}{r_j,*}_{\pr_z, j}$ 
performed on any of the ranked registers, for $1\leq j\leq k$,
the highest rank for $j$ at the time of the write was $r_j$. 

Finally consider the execution $\Delta\EX''$ that is similar to 
$\EX''$ without containing $\wrt_1$. In other words $\Delta\EX''$
extends $\EX$ with the write operation $\wrt_2$. Observe that any 
write operation $\rrw{r'}{r_j, *}_{\pr_z, j}$ performed by $\pr_z$ on 
ranked register $j$ during $\wrt_2$ observes a highest rank $r_j$ 
as in $\EX''$. So if such a write committed (or aborted) in $\EX''$ 
will also commit (or abort) in $\Delta\EX''$ as well. Therefore,
since $\wrt_2$ revised the value of the traceable register in $\EX''$ 
will revise the value of the traceable register in $\Delta\EX''$ 
as well. However the last state of the traceable register in $\EX$ 
is $(v,ver)$ and the value $\wrt_2$ revises is associated with 
a version $ver'\neq ver$. Thus $\Delta\EX''$ contains an illegal 
transition for a traceable object and hence contradicts our 
initial assumption.  

\noindent{\bf Direction 2:}
Here we need to show that if a write operation 
$\rrw{r}{*,commit}_{{\pr_i},j}$ on some ranked register $j$ commits, then the write 
$\wrt_1 = \trw{ver}{ver',mod}_{\pr_i}$
revises the value of the traceable register. 
Let us consider the negation of the above sentence.
In other words, if all the write operations performed 
on the ranked register during $\wrt_1$ abort, then $\wrt_1$
does not revise the value of the register. 
Assume to derive contradiction that if all the 
write operations on the rank register abort, then 
$\wrt_1$ revises the value of the traceable register. 

We extend now $\EX$ with $\wrt_1$ to obtain $\EX'$.
Since all the write operations 
performed during $\wrt_1$ abort it follows that 
$\forall \rrw{r}{r_j,abort}_{{\pr_i},j}$, that performed
during $\wrt_1$, $r_j>r$, where $r_j$ the highest rank 
of register $j$. Assume that the last state of $\EX'$ 
is associated with version $ver'$, with $ver'\neq ver$.

Let now extend $\EX'$ with another write operation 
$\wrt_2=\trw{ver}{*}_{\pr_z}$. Since $ver\neq ver'$ then 
by traceability $\wrt_2$ does not revise the value 
of the traceable register. So, by our assumption 
there must exists some ranked register, say $j\in[1,k]$, 
such that the write operation $\rrw{r}{*,commit}_{\pr_z, j}$ 
commits. Note that for the highest rank on the ranked register
$j$ when this write is executed is $r_j$. 

Consider now an execution $\Delta\EX''$ that is similar 
to $\EX''$ but it does not contain $\wrt_1$. In other 
words we obtain $\Delta\EX''$ by extending 
$\EX$ with the write operation $\wrt_2$. Notice 
that every write operation $\rrw{r}{r_j,*}_{\pr_z,j}$
observes the same highest rank $r_j$ as in $\EX''$.
Thus, if a write $\rrw{r}{r_j,*}_{{\pr_z},j}$ committed 
in  $\EX''$, commits in $\Delta\EX''$ as well. Thus,
$\wrt_2$ cannot distinguish $\Delta\EX''$ from $\EX''$ 
and hence it does not revise the value in $\Delta\EX''$ either. 

However $\wrt_2$ is not concurrent with any other operation 
and uses its version is equal to the version of the last 
state in $\EX$, $ver$. By traceability transitions, 
such write operation should have revised the value of 
the object and this leads us to contradiction.
\end{proof}

The next lemma shows that if an operation $\op_2$ does not change 
the version of the traceable register and returns a version 
generated by an operation $\op_1$, then $\op_2$ must write 
to some ranked register that $\op_1$ written with a rank 
smaller than the one used by $\op_1$.

\begin{lemma}
\label{lem:rrabort}
Let $\op_1 = \trw{ver}{ver_1,success}_{\pr_i}$ and 
$\op_2 = \trw{ver_1}{ver_2,abort}_{\pr_z}$
two write operations that appear in an execution $\EX$ s.t. 
$\op_1\bef_{\EX}\op_2$.
%, and cause the transitions 
%$\delta_1 = \tup{(v,ver_1), (\op_1,ver_1), (v_1,ver')}$ and 
%$\delta_2 = \tup{(v_1,ver'), (\op_2,ver_2), (v_1,ver')}$ 
%respectively. 
There exists some shared register $j$ such that 
$\pr_i$ performs an $\rrw{r}{*,commit}_{\pr_i,j}$ during $\op_1$, 
and $\pr_z$ performs an $\rrw{r'}{*,abort}_{\pr_z,j}$ during $\op_2$, and $r > r'$.
\end{lemma}
%% Abort Proof
\begin{proof}
We will assume to derive contradiction that $\op_2$ does not write on any 
ranked register that $\pr_i$ wrote (and committed) during $\op_1$. 
More formally, let $R_1$ be the set of ranked registers
s.t. for all $j\in R_1$, $\rrw{r}{*,commit}_{\pr_i,j}$ for some rank 
$r$ during $\op_1$.  Let $R_2$ be the set of ranked registers 
s.t. for all $q\in R_2$, $\pr_z$ invokes $\rrw{r'}{*,abort}_{\pr_z,q}$ 
during $\op_2$. Note that since $\op_2$ does not change the version 
of the object, then according to Lemma \ref{lem:commit}, 
no ranked register commits during $\op_2$ and hence $R_2$ contains
all the ranked registers that $\pr_z$ tried to write to.  
According to our assumption $R_1\cap R_2 = \emptyset$. 

Let us construct an execution that contain the two operations $\op_1$ and $\op_2$.
Consider an execution fragment $\EX$ that ends with a state associated with a version $ver$. 
Let us assume that there exists an algorithm that uses $k$ ranked registers 
each with a highest rank $r_1, r_2,\ldots,r_k$ respectively at the end of $\EX$. 
%
We extend $\EX$ with operation $\op_1$ and obtain $\EX_1$. Since $\op_1$ 
changes the version of the object, according to Lemma \ref{lem:commit},
there exists a ranked register $j\in R_1$ such that, 
$\rrw{r}{*,commit}_{\pr_i,j}$ during $\op_1$. 

Next we extend $\EX_1$ by $\op_2$ and obtain $\EX_2$. 
Notice that $\op_2$ does not change the value of the traceable 
register and thus, by Lemma \ref{lem:commit}, for all the ranked 
registers $j\in R_2$, $\rrw{r'}{r_h,abort}_{\pr_z,j}$. Since 
according to our assumption, $R_1\cap R_2=\emptyset$, then it 
must be the case that the highest rank observed by $\op_2$ in any
$j\in R_2$ is $r_h=r_j$, i.e. the highest rank of $j$ at the end of $\EX$.
That includes also the ranked registers that aborted when 
$\pr_i$  tried to modify during $\op_1$.

Consider now the execution $\Delta\EX_2$ which is obtained 
by extending $\EX$ with $\op_2$. Notice that since $\pr_z$
does not communicate with $\pr_i$ then it communicates with 
the same set $R_2$ of ranked registers. Every write operation 
on the ranked registers $j\in R_2$ return the same highest
rank an in $\EX_2$. So $\op_2$ cannot distinguish $\EX_2$ 
from $\Delta\EX_2$ and thus returns the same version of the object. 
However, this violates the validity condition of
weak traceability since $\op_2$ returns a version $ver_1$ 
that is not yet reached by the object. Thus, this contradicts 
our assumption and the lemma follows. 
\end{proof}

Next we show that if two succeeding operation $\op_1, \op_2$ 
change the version of the traceable register, they both 
performed a committed write on at least a single common ranked register.
In other words if an operation changes a version $ver$ it 
has to write in at least one ranked register that the operation
that introduced $ver$ wrote on. 

\begin{lemma}
\label{lem:rrcommon}
Let $\op_1 = \trw{ver}{ver_1,success}_{\pr_i}$ and 
$\op_2 = \trw{ver_1}{ver_2,success}_{\pr_z}$
two write operations that appear in an execution $\EX$ s.t. 
$\op_1\bef_{\EX}\op_2$.
%, and cause the transitions 
%$\delta_1 = \tup{(v,ver_1), (\op_1,ver_1), (v_1,ver')}$ and 
%$\delta_2 = \tup{(v_1,ver'), (\op_2,ver_2), (v_1,ver')}$ 
%respectively. 
There exists some shared register $j$ such that 
$\pr_i$ performs an $\rrw{r}{*,commit}_{\pr_i,j}$ during $\op_1$, 
and $\pr_z$ performs an $\rrw{r'}{*,commit}_{\pr_z,j}$ during $\op_2$.
%, and $r > r'$.
\end{lemma}

\begin{proof}
This proof follow similar techniques as Lemma \ref{lem:rrabort}.
We will assume to derive contradiction that $\op_2$ does not write on any 
ranked register that $\pr_i$ wrote (and committed) during $\op_1$. 
More formally, let $R_1$ be the set of ranked registers
s.t. for all $j\in R_1$, $\rrw{r}{*,commit}_{\pr_i,j}$ for some rank 
$r$ during $\op_1$.  Let $R_2$ be the set of ranked registers 
s.t. for all $q\in R_2$, $\pr_z$ invokes $\rrw{r'}{*,commit}_{\pr_z,q}$ 
during $\op_2$. Note that since both $\op_1$ and $\op_2$ change the version 
of the object, then according to Lemma \ref{lem:commit}, 
then $|R_1|,|R_2| \geq 1$.  
According to our assumption $R_1\cap R_2 = \emptyset$. 

We can now construct an execution $\EX_2$ that contains $\op_1\bef_{\hist{\EX_2}}\op_2$.
Let $\pr_i$ perform $\rrw{r}{*,commit}_{\pr_i,x}$ for all 
ranked register $x\in R_1$ during $\op_1$, and $\pr_z$ perform
$\rrw{r'}{r_h,commit}_{\pr_z,y}$ for all 
ranked register $y\in R_2$ during $\op_1$. Since $R_1\cap R_2=\emptyset$,
then every ranked write from $\pr_z$ at $q\in R_2$ observes a highest 
$r_h=r_q$. 

If we consider next an execution $\Delta\EX_2$ that is similar with $\EX_2$ 
but without containing $\op_1$, with similar arguments as in Lemma \ref{lem:rrabort}
we can show that $\op_2$ cannot distinguish the two executions. So 
$\op_2$ revises $ver_1$ in $\Delta\EX_2$ as well. However, $ver_1$ wan
never introduced in $\Delta\EX_2$, therefore $\op_2$ violates the validity
condition of traceability. This contradicts our assumption.~\end{proof}     
%
%
%Let us construct an execution that contain the two operations $\op_1$ and $\op_2$.
%Consider an execution fragment $\EX$ that ends with a state associated with a version $ver$. 
%Let us assume that there exists an algorithm that uses $k$ ranked registers 
%each with a highest rank $r_1, r_2,\ldots,r_k$ respectively at the end of $\EX$. 
%%
%We extend $\EX$ with the operation $\op_1$ and obtain $\EX_1$. Since $\op_1$ 
%changes the version of the object, according to Lemma \ref{lem:commit},
%there exists a ranked register $j\in R_1$ such that, 
%$\rrw{r}{*,commit}_{\pr_i,j}$ during $\op_1$. 
%
%Next we extend $\EX_1$ by $\op_2$ and obtain $\EX_2$. 
%Notice that $\op_2$ also changes the value of the traceable 
%register and thus, by Lemma \ref{lem:commit}, there exists a rank 
%register $j\in R_2$, $\rrw{r'}{r_h,commit}_{\pr_z,j}$. Since 
%according to our assumption, $R_1\cap R_2=\emptyset$, then it 
%must be the case that the highest rank observed by $\op_2$ in any
%$j\in R_2$ is $r_h=r_j$, i.e. the highest rank of $j$ at the end of $\EX$.
%That includes also the ranked registers that aborted when 
%$\pr_i$ tried to modify during $\op_1$.
%
%Consider now the execution $\Delta\EX_2$ which is obtained 
%by extending $\EX$ with $\op_2$. Notice that since $\pr_z$
%does not communicate with $\pr_i$ then it communicates with 
%the same set $R_2$ of ranked registers. Every write operation 
%on the ranked registers $j\in R_2$ return the same highest
%rank an in $\EX_2$. So $\op_2$ cannot distinguish $\EX_2$ 
%from $\Delta\EX_2$ and thus returns the same version of the object. 
%However, this violates the validity condition of
%weak traceability since $\op_2$ revises a version $ver_1$ 
%that is not yet reached by the object. Thus, this contradicts
%our assumption and the lemma follows. 


Using now Lemmas \ref{lem:rrabort} and \ref{lem:rrcommon}
we can show that an operation that changes the version of 
the traceable object must use a rank higher than any previously
successful operation.

\begin{lemma}
\label{lem:rrorder}
In any execution $\EX$ if $\op_1 = \trw{ver}{ver_1,success}_{\pr_i}$ and 
$\op_2 = \trw{ver_1}{ver_2,success}_{\pr_z}$, s.t. 
$\op_1\bef_{\EX}\op_2$, then there exists some shared register $j$ such that 
$\pr_i$ performs an $\rrw{r}{*,commit}_{\pr_i,j}$ during $\op_1$, 
and $\pr_z$ performs an $\rrw{r'}{*,commit}_{\pr_z,j}$ during $\op_2$, and $r' > r$.
\end{lemma}

\begin{proof}
	Assume to derive contradiction that we can have such two operations
	but $r' < r$. Note that this does not violate the definition of the
	ranked registers. 
	
	Consider an execution $\EX$ that ends with a version $ver$.
	We extend $\EX$ with the following non-concurrent operations 
	to obtain execution $\EX_1$:
	\begin{itemize}
		\item operation $\op_1 = \trop{ver}{ver_1,success}_{\pr_i}$
		\item operation $\op_2 = \trop{ver}{ver_1,fail}_{\pr_z}$
		\item operation $\op_3 = \trop{ver_1}{ver_2,success}_{\pr_q}$
	\end{itemize}
	According to Lemmas \ref{lem:rrabort} and \ref{lem:rrcommon}, there should 
	exists a ranked register $j$ such that all three operations perform a write 
	operation. The two operations $\op_1$ and $\op_3$ perform a committed write
	on $j$, whereas $\op_2$ performs an aborted write on $j$. According to our assumption
	let $\rrw{r_1}{r_j,commit}_{\pr_i,j}$ be the write from $\pr_i$, followed 
	by a $\rrw{r_2}{r_1,abort}_{\pr_z,j}$ from $\pr_z$, and a 
	$\rrw{r_3}{r_1,commit}_{\pr_q,j}$ from $\pr_q$. Notice that
	$r_2 < r_1$, by Lemma \ref{lem:rrabort}, and $r_3<r_1$ according
	to our assumption. Also assume w.l.o.g. that $r_3 < r_m$, for 
	$m\neq j$ and $1\leq m\leq k$. Notice that the write from $\pr_q$ 
	does not violate the ranked register definition, as a write operation
	with a smaller rank does not have to abort. So in order to preserve 
	traceability $\op_3$ needs to change the version $ver_1$.
	
	Consider now the execution $\Delta\EX_1$ that contains the same 
	three operation but with $\op_2$ and $\op_3$ in reverse order. 
	In particular $Rev\EX_1$ extends $\EX$ with operations:
	\begin{itemize}
		\item operation $\op_1 = \trop{ver}{ver_1,success}_{\pr_i}$
		\item operation $\op_3 = \trop{ver_1}{ver_2,success}_{\pr_q}$
		\item operation $\op_2 = \trop{ver}{ver_1,fail}_{\pr_z}$
	\end{itemize}  
	Observe now that, according to Lemma \ref{lem:commit}, all the
	write operations that $\op_2$ performed in $\EX_1$ aborted. Thus,
	$\op_3$ observes the same ranks from any $\rrw{r_3}{*,abort}_{\pr_q,j}$
	it performs, and hence it cannot distinguish $\Delta\EX_1$ from $\EX_1$. 
	Therefore, it revises $ver_1$ in $\Delta\EX_1$ as well. When $\op_2$ 
	is invoked it performs again an $\rrw{r_2}{r_h,*}_{\pr_z,j}$ on 
	ranked register $j$. Since however, according to our assumption, $r_3< r_1$,
	then $\pr_z$ observes the highest rank on $j$ to be $r_h=r_1$. Also 
	since $r_3$ is smaller than any other rank $r_m$, for $m\neq j$ and $1\leq m\leq k$,
	then $\pr_z$ observes a highest rank $r_h=r_m$ for any other 
	$\rrw{r_2}{r_h,*}_{\pr_z,m}$ it performs. Hence, $\op_2$ cannot 
	distinguish $\Delta\EX_1$ from $\EX_1$ either so it does not 
	change the version returning version $ver_1$ and failing. 
	This however violates the consolidation property of traceability and 
	leads to contradiction. 
\end{proof}

Next we present out main result that shows that a traceable 
register cannot be implemented with ranked registers as those
were defined in \cite{GD05}.

\begin{theorem}
There is no algorithm that implements a traceable register 
using a set of ranked registers. 
\end{theorem}

\begin{proof}
	From Lemma \ref{lem:rrorder} it follows that for every two executions $\op_1,\op_2$, such that
	$\op_2$ revises the version that $\op_1$ produces then, if $\op_1$ uses a 
	rank $r_1$, $\op_2$ should use a rank $r_2$ s.t. $r_1 < r_2$. By the definition 
	of a ranked register a write operation may commit even $r_1 > r_2$. Since 
	according to Lemma \ref{lem:commit} both $\op_1$ and $\op_2$ need to commit,
	and since by Lemma \ref{lem:rrcommon} need to commit to at least a common 
	rank register, then using ranks $r_1 < r_2$ would violate traceabiility by 
	Lemma \ref{lem:rrorder} and the theorem follows.  
%	
%	From Lemma \ref{lem:rrcommon} it is clear that if an operation
%	produces a version $ver_i$, s.t. 
%	$\op_1 = \trop{ver_{i-1}}{ver_i,success}_{\pr_i}$, and some 
%	succeeding operation $\op_2 = \trop{ver_i}{ver_{i+1},success}_{\pr_j}$
%	revises $ver_i$ it must be the case that there is at least 
%	a single ranked register $r$ s.t. $\pr_i$ invokes a $\rrw{r_1}{*,commit}_{\pr_i,r}$
%	during $\op_1$ and $\pr_j$ invokes a $\rrw{r_2}{*,commit}_{\pr_j,r}$
%	during $\op_2$. From Lemma \ref{lem:rrorder} it follows that $r_1 < r_2$. 
%	We also know from traceability definition that $ver_{i-1} < ver_i$.
%	
\end{proof}

%Notice that a stronger definition of rank registers, one that requires that 
%an operation always aborts if it discovers a smaller previous rank, may have 
%been sufficient to implement traceable registers.  

